Finding and Visualizing Weaknesses of Deep Reinforcement Learning Agents

As deep reinforcement learning driven by visual perception becomes more widely used there is a growing need to better understand and probe the learned agents. Understanding the decision making process and its relationship to visual inputs can be very valuable to identify problems in learned behavior. However, this topic has been relatively under-explored in the research community. In this work we present a method for synthesizing visual inputs of interest for a trained agent. Such inputs or states could be situations in which specific actions are necessary. Further, critical states in which a very high or a very low reward can be achieved are often interesting to understand the situational awareness of the system as they can correspond to risky states. To this end, we learn a generative model over the state space of the environment and use its latent space to optimize a target function for the state of interest. In our experiments we show that this method can generate insights for a variety of environments and reinforcement learning methods. We explore results in the standard Atari benchmark games as well as in an autonomous driving simulator. Based on the efficiency with which we have been able to identify behavioural weaknesses with this technique, we believe this general approach could serve as an important tool for AI safety applications.

==> figures/fig_filters.tex <==
\begin{figure*}
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{.48\linewidth}
  \includegraphics[width=\linewidth]{images/filters_pong.png}
  \caption{Pong}
\end{subfigure}\hfill
\begin{subfigure}[b]{.48\linewidth}
  \includegraphics[width=\linewidth]{images/filters_alien.png}
  \caption{Alien}
\end{subfigure}

\begin{subfigure}[b]{.48\linewidth}
  \includegraphics[width=\linewidth]{images/filters_seaquest.png}
  \caption{Sea Quest}
\end{subfigure}\hfill
\begin{subfigure}[b]{.48\linewidth}
  \includegraphics[width=\linewidth]{images/filters_yarsrevenge.png}
  \caption{Yar's Revenge}
\end{subfigure}

\begin{subfigure}[b]{.48\linewidth}
  \includegraphics[width=\linewidth]{images/filters_krull.png}
  \caption{Krull}
\end{subfigure}\hfill
\begin{subfigure}[b]{.48\linewidth}
  \includegraphics[width=\linewidth]{images/filters_namethisgame.png}
  \caption{Name This Game}
\end{subfigure}
\caption{\textbf{Conv1 Weights DQN.} We display the weights of the first layer of DQNs trained on several Atari games. Columns represent the 32 different $8\times 8$ filters, while the four rows correspond the to four frames that are stacked as an input for the network. The vertically stacked weights represent the temporal component with the current frame at the bottom and frame $t-3$ at the top.}
\label{fig:filters}
\end{figure*}

==> figures/fig_vaes.tex <==
\begin{figure}
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{.2\textwidth}
  \includegraphics[width=\linewidth]{images/pong_ori.png}
  \caption{Input}
\end{subfigure}\hfill
\begin{subfigure}[b]{.2\textwidth}
  \includegraphics[width=\linewidth]{images/pong_rec_vanilla.png}
  \caption{Vanilla VAE}
\end{subfigure}\hfill
\begin{subfigure}[b]{.2\textwidth}
  \includegraphics[width=\linewidth]{images/pong_rec_mask.png}
  \caption{$\mathcal{L}_p$ only}
\end{subfigure}\hfill
\begin{subfigure}[b]{.2\textwidth}
  \includegraphics[width=\linewidth]{images/pong_rec_full.png}
  \caption{$\mathcal{L}_p$ + $\mathcal{L}_a$ (ours)}
\end{subfigure}
\caption{\textbf{Visual Comparison of Losses.} We show input a), and reconstructions b-d) using different loss terms. Vanilla VAE is blurry around the ball and paddle. Even though c) and d) are similar, the fact that performance differs (Table \ref{tab:losses}) shows the agent's sensitivity. (best viewed digitally)}
\label{fig:vaes}
\end{figure}
